PROD: Progressive Distillation for Dense Retrieval

Knowledge distillation is an effective way to transfer knowledge from a strong teacher to an efficient student model. Ideally, we expect the better the teacher is, the better the student. However, this expectation does not always come true. It is common that a better teacher model results in a bad student via distillation due to the nonnegligible gap between teacher and student. To bridge the gap, we propose PROD, a PROgressive Distillation method, for dense retrieval. PROD consists of a teacher progressive distillation and a data progressive distillation to gradually improve the student. We conduct extensive experiments on five widely-used benchmarks, MS MARCO Passage, TREC Passage 19, TREC Document 19, MS MARCO Document and Natural Questions, where PROD achieves the state-of-the-art within the distillation methods for dense retrieval. The code and models will be released.

==> tables/ablation_bak.tex <==
\begin{table*}[ht]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{Variant}                                   & \textbf{MRR@10} & \textbf{R@1} & \textbf{R@5} & \textbf{R@20} & \textbf{R@50} & \textbf{R@100} & \textbf{R@1k} \\ \hline
\textbf{6-layer DE} & 31.66           & 20.14        & 47.45        & 68.95         & 79.99         & 85.59          & 96.19         \\ \hline
\textbf{12-layer DE $\rightarrow$ 6-layer DE}                             & 35.69           & 23.65        & 52.54        & 73.94         & 84.09         & 89.31          & 97.59         \\
* 12-layer CE $\rightarrow$ 6-layer DE                             & 37.44           & 25.11        & 54.11        & 75.03         & 84.44         & 88.81          & 97.15         \\
* 24-layer CE $\rightarrow$ 6-layer DE                             & 36.18           & 23.80        & 53.08        & 74.57         & 84.15         & 89.13          & 97.46         \\ \hline
\textbf{12-layer CE + 12-layer DE $\rightarrow$ 6-layer DE}               & 38.09           & 25.34        & 55.54        & 76.75         & 86.12         & 90.83          & 97.72         \\
* 12-layer DE + 12-layer CE $\rightarrow$ 6-layer DE & 34.90 & 22.98 & 51.07 & 73.01 & 82.95 & 88.44 & 97.22 \\
* 24-layer CE + 12-layer DE $\rightarrow$ 6-layer DE               & 38.08           & 25.46        & 55.46        & 76.76         & 85.72         & 90.53          & 97.82         \\ \hline
\textbf{24-layer CE + 12-layer CE + 12-layer DE $\rightarrow$ 6-layer DE} & 38.75           & 25.89        & 55.86        & 77.68         & 86.56         & 91.33          & 98.41         \\ 
* 24-layer CE + 12-layer CE + 12-layer CE $\rightarrow$ 6-layer DE & 38.29	& 25.87 & 55.14 & 75.64 & 84.58 & 88.62 & 96.40 \\
* 12-layer CE + 12-layer CE + 12-layer DE $\rightarrow$ 6-layer DE & 37.88 & 24.94 & 55.53 & 76.62 & 86.12 & 90.76 & 98.01 \\
* 24-layer CE + 24-layer CE + 12-layer DE $\rightarrow$ 6-layer DE & 37.63 & 24.87 & 54.99 & 76.39 & 85.54 & 90.26 & 98.07 \\ \hline
\textbf{PROD}                                               & 39.34           & 26.66        & 56.35        & 78.09         & 87.06         & 91.52          & 98.44         \\ \hline
% \begin{table*}[ht]
% \small
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{l|cccc}
\hline
\textbf{Method} & \textbf{R@1} & \textbf{R@5} & \textbf{R@20} & \textbf{R@100} \\ \hline
 \textbf{6-layer DE} & 45.96 & 67.76 & 78.88 & 86.24         \\ \hline
\textbf{12-layer DE $\rightarrow$ 6-layer DE} & 54.82 & 73.73 & 82.70 & 88.29 \\
* 12-layer CE $\rightarrow$ 6-layer DE & 52.16 & 71.54 & 81.78 & 88.24 \\
* 24-layer CE $\rightarrow$ 6-layer DE & 51.19 & 70.57 & 80.62 & 87.15 \\ \hline
\textbf{12-layer CE + 12-layer DE $\rightarrow$ 6-layer DE} & 57.12 & 75.12 & 84.30 & 88.82 \\
* 24-layer CE + 12-layer DE $\rightarrow$ 6-layer DE & 56.87 & 74.75 & 84.22 & 88.81    \\ \hline

\textbf{24-layer CE + 12-layer CE + 12-layer DE $\rightarrow$ 6-layer DE} & 57.20 & 75.54 & 84.66 & 89.48         \\  \hline
\textbf{PROD} & 57.63 & 75.61 & 84.72 & 89.56       \\ \hline
% \end{tabular}
% % }
% \caption{The results on NQ.}
% \label{tab:NQAblation}
% \end{table*}
\end{tabular}
}
\caption{The results of ablation study on \textsc{MS-Pas}.}
\label{tab:MSPasAblation}
\end{table*}





\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|l|ccccccc}
\hline
\textbf{Retriever} & \textbf{Ranker} & \textbf{MRR@10} & \textbf{R@1} & \textbf{R@5} & \textbf{R@20} & \textbf{R@50} & \textbf{R@100} & \textbf{R@1k} \\ \hline
12-layer DE & - & 35.77 &	23.50 & 52.72 & 74.18 & 84.10 & 89.14 & 97.61 \\
12-layer DE & 12-layer CE & 40.81 & 27.88 & 58.58 & 79.04 & 86.52 & 90.81 & 97.61 \\
12-layer DE & 24-layer CE & 41.96 & 28.84 & 59.81 & 80.00 & 87.89 & 92.23 & 97.61 \\ \hline
\end{tabular}
\caption{The performance of three kinds of teacher models in the first step on MS Pas}
\label{tab:MSPasRerank}
\end{table*}





\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|l|cccc}
\hline
\textbf{Retriever} & \textbf{Ranker} & \textbf{R@1} & \textbf{R@5} & \textbf{R@20} & \textbf{R@100} \\ \hline
12-layer DE & - &  52.94 & 73.15 & 82.70 & 88.68 \\
12-layer DE & 12-layer CE & 60.38 & 79.46 & 86.02 & 88.68 \\
12-layer DE & 24-layer CE & 64.78 & 80.57 & 86.24 & 88.68 \\ \hline
\end{tabular}
\caption{The performance of three kinds of teacher models in the first step on NQ}
\label{tab:NQRerank}
\end{table*}


\begin{table*}[ht]
\small
\centering
\begin{tabular}{l|ccccccc}
\hline
\textbf{Retriever} & \textbf{MRR@10} & \textbf{R@1} & \textbf{R@5} & \textbf{R@20} & \textbf{R@50} & \textbf{R@100} & \textbf{R@1k} \\ \hline
2-layer DE & 27.31 &	17.18 & 40.83 & 61.65 & 72.79 & 79.79 & 93.57 \\
12-layer DE $\rightarrow$ 2-layer DE  & 30.78 & 19.27 & 46.48 & 67.87 & 78.88 & 85.32 & 96.29 \\
12-layer CE + 12-layer DE $\rightarrow$ 2-layer DE  & 34.10 & 22.41 & 50.59 & 71.15 & 80.62 & 86.32 & 95.56 \\
24-layer CE + 12-layer DE $\rightarrow$ 2-layer DE  & 32.92 &	21.68 & 48.47 & 69.84 & 80.24 & 85.95 & 95.49 \\ \hline
\end{tabular}
\caption{The results of distilling on 2-layer DE using 12-layer CE or 24-layer CE in the second step of PROD, on MS Pas.}
\label{tab:MSPas2layer}
\end{table*}

==> tables/zero_shot_results.tex <==
\begin{table*}[t!]
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{l | c c c c | c c c | c c c}
\hline
\multicolumn{1}{l|}{\textbf{Model ($\rightarrow$)}} &
\multicolumn{4}{c|}{\textbf{Sparse}}   &
\multicolumn{3}{c|}{\textbf{Dense}} &
\multicolumn{3}{c}{\textbf{Ours}} \\ 
\hline
\textbf{Dataset ($\downarrow$)} &
\textbf{BM25} &
\textbf{DeepCT} &
\textbf{SPARTA} &
\textbf{docT5query} &
\textbf{DPR} &
\textbf{ANCE} &
\textbf{TAS-B} &
\textbf{Baseline1} &
\textbf{Baseline2} &
\textbf{\textsc{ProD}} \\ \hline

MS MARCO & 0.228 & 0.296$^\ddagger$ & 0.351$^\ddagger$ & 0.338$^\ddagger$ & 0.177 & 0.388$^\ddagger$ & 0.408$^\ddagger$ & - & - & 0.713 \\ \hline \hline

TREC-COVID    & 0.656 & 0.406 & 0.538 & \underline{0.713} & 0.332& 0.654 & 0.481 & - & - & 0.674 \\
BioASQ        & 0.465 & 0.407 & 0.351 & \textcolor{black}{0.431} & 0.127 & 0.306 & 0.383 & - & - & - \\
NFCorpus      & 0.325 & 0.283 & 0.301 & \underline{0.328} & 0.189 & 0.237 & 0.319 & - & - & 0.314 \\ \hline
NQ            & 0.329 & 0.188 & 0.398 & 0.399 & 0.474$^\ddagger$ & 0.446 & 0.463 & - & - & 0.529 \\ 
HotpotQA      & \underline{0.603} & 0.503 & 0.492 & 0.580 & 0.391 & 0.456 & 0.584 & - & - & 0.571 \\ 
FiQA-2018     & 0.236 & 0.191 & 0.198 & 0.291 & 0.112 & 0.295 & 0.300 & - & - & 0.308 \\ \hline
Signal-1M (RT)& \underline{0.330} & 0.269 & 0.252 & 0.307 & 0.155 & 0.249 & 0.289 & - & - & - \\ \hline
TREC-NEWS     & 0.398 & 0.220 & 0.258 & \underline{0.420} & 0.161 & 0.382 & 0.377 & - & - & - \\
Robust04     & 0.408 & 0.287 & 0.276 & \underline{0.437} & 0.252 & 0.392 & 0.427 & - & - & - \\ \hline
ArguAna       & 0.315 & 0.309 & 0.279 & 0.349 & 0.175& 0.415 & \underline{0.429} & - & - & 0.377 \\  
Touch\'e-2020 & \textbf{0.367} & 0.156 & 0.175 & \underline{0.347} & 0.131 & 0.240 & 0.162 & - & - & 0.306 \\ \hline 
CQADupStack   & 0.299 & 0.268 & 0.257 & 0.325 & 0.153 & 0.296 & 0.314 & - & - & 0.300 \\
Quora         & 0.789 & 0.691 & 0.630 & 0.802 & 0.248 & \underline{0.852} & 0.835 & - & - & 0.781 \\ \hline
DBPedia       & 0.313  & 0.177 & 0.314 & 0.331 & 0.263 & 0.281 & 0.384 & - & - & 0.386 \\ \hline
SCIDOCS       & 0.158 & 0.124 & 0.126 & \underline{0.162} & 0.077 & 0.122 & 0.149 & - & - & 0.132 \\ \hline
FEVER         & 0.753 & 0.353 & 0.596 & \textcolor{black}{0.714} & 0.562& 0.669 & 0.700 & - & - & 0.745 \\ 
Climate-FEVER & 0.213 & 0.066 & 0.082 & 0.201 & 0.148 & 0.198 & \underline{0.228} & - & - & 0.217 \\ 
SciFact       & 0.665 & 0.630 & 0.582 & \underline{0.675} & 0.318 & 0.507 & 0.643 & - & - & 0.603 \\ \hline
% \multicolumn{2}{c|}{Avg. Performance vs. BM25} & \textbf{- 27.9\%} & \textbf{- 20.3\%} & \textbf{+ 1.6\%} & \textbf{- 47.7\%} & \textbf{- 7.4\%} & \textbf{ - 2.8\%} & - & - & - \\ 
% \hline
\end{tabular}
}
\caption{In-domain and zero-shot nDCG@10 scores on \textsc{beir} benchmark.
The best score on a given dataset is marked in \textbf{bold}, and the second best is \underline{underlined}.
$\ddagger$ indicates the in-domain performances.}
\label{tab:zero_shot_ndcg}
\end{table*}


% \begin{table*}[t!]
% \small
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l | c c c c | c c c | c c c}
% \hline
% \multicolumn{1}{l|}{\textbf{Model ($\rightarrow$)}} &
% \multicolumn{4}{c|}{\textbf{Sparse}}   &
% \multicolumn{3}{c|}{\textbf{Dense}} &
% \multicolumn{3}{c}{\textbf{Ours}} \\ 
% \hline
% \textbf{Dataset ($\downarrow$)} &
% \textbf{BM25} &
% \textbf{DeepCT} &
% \textbf{SPARTA} &
% \textbf{docT5query} &
% \textbf{DPR} &
% \textbf{ANCE} &
% \textbf{TAS-B} &
% \textbf{Baseline1} &
% \textbf{Baseline2} &
% \textbf{\textsc{ProD}} \\ \hline

% MS MARCO      & 0.658 & 0.752$^\ddagger$ & 0.793$^\ddagger$ & 0.819$^\ddagger$ & 0.552 & 0.852$^\ddagger$ & \textbf{0.884$^\ddagger$} & - & - & - \\ \hline \hline

% TREC-COVID    & \underline{0.498} & 0.347 & 0.409 & \textbf{0.541} & 0.212 & 0.457 & 0.387 & - & - & - \\
% BioASQ        & \textbf{0.714} & \underline{0.699} & 0.351 & 0.646 & 0.256 & 0.463 & 0.579 & - & - & - \\
% NFCorpus      & 0.250 & 0.235 & 0.243 & 0.253 & 0.208 & 0.232 & \textbf{0.280} & - & - & - \\ \hline
% NQ            & 0.760 & 0.636 & 0.787 & 0.832 & 0.880$^\ddagger$ & 0.836 & \underline{0.903} & - & - & - \\ 
% HotpotQA      & \underline{0.740} & 0.731 & 0.651 & 0.709 & 0.591 & 0.578 & 0.728 & - & - & - \\ 
% FiQA-2018     & 0.539 & 0.489 & 0.446 & 0.598 & 0.342 & 0.581 & 0.593 & - & - & - \\ \hline
% Signal-1M (RT)& \textbf{0.370} & 0.299 & 0.270 & \underline{0.351} & 0.162 & 0.239 & 0.304 & - & - & - \\ \hline
% TREC-NEWS     & \underline{0.422} & 0.316 & 0.262 & \textbf{0.439} & 0.215 & 0.398 & 0.418 & - & - & - \\
% Robust04      & \textbf{0.375} & 0.271 & 0.215 & \underline{0.357} & 0.211 & 0.274 & 0.331 & - & - & - \\ \hline
% ArguAna       & 0.942 & 0.932 & 0.893 & \underline{0.972} & 0.751 & 0.937 & 0.942 & - & - & - \\  
% Touch\'e-2020 & \underline{0.538} & 0.406 & 0.381 & \textbf{0.557} & 0.301 & 0.458 & 0.431 & - & - & - \\ \hline 
% CQADupStack   & 0.606 & 0.545 & 0.521 & \underline{0.638} & 0.403 & 0.579 & 0.622 & - & - & - \\
% Quora         & 0.973 & 0.954 & 0.896 & 0.982 & 0.470 & 0.987 & 0.986 & - & - & - \\ \hline
% DBPedia       & 0.398 & 0.372 & 0.411 & 0.365 & 0.349 & 0.319 & \textbf{0.499} & - & - & - \\ \hline
% SCIDOCS       & \underline{0.356} & 0.314 & 0.297 & \textbf{0.360} & 0.219 & 0.269 & 0.335 & - & - & - \\ \hline
% FEVER         & 0.931 & 0.735 & 0.843 & 0.916 & 0.840 & 0.900 & \textbf{0.937} & - & - & - \\ 
% Climate-FEVER & 0.436 & 0.232 & 0.227 & 0.427 & 0.390 & 0.445 & \textbf{0.534} & - & - & - \\  
% SciFact       & \underline{0.908} & 0.893 & 0.863 & \textbf{0.914} & 0.727 & 0.816 & 0.891 & - & - & - \\ \hline
% \end{tabular}
% }
% \caption{In-domain and zero-shot R@100 scores on \textsc{beir} datasets.
% We show capped R@100 scores on TREC-COVID.
% The best score on a given dataset is marked in \textbf{bold}, and the second best is \underline{underlined}.
% $\ddagger$ indicates in-domain retrieval performance.}
% \label{tab:zero_shot_recall}
% \end{table*}
